Distributed Computations in Fully-Defective Networks

We address fully-defective asynchronous networks, in which all links are subject to an unlimited number of alteration errors, implying that all messages in the network may be completely corrupted. Despite the possible intuition that such a setting is too harsh for any reliable communication, we show how to simulate any algorithm for a noiseless setting over any fully-defective setting, given that the network is 2-edge connected. We prove that if the network is not 2-edge connected, no non-trivial computation in the fully-defective setting is possible. The key structural property of 2-edge-connected graphs that we leverage is the existence of an oriented (non-simple) cycle that goes through all nodes [Robbins, 1939]. The core of our technical contribution is presenting a construction of such a Robbins cycle in fully-defective networks, and showing how to communicate over it despite total message corruption. These are obtained in a content-oblivious manner, since nodes must ignore the content of received messages.

==> images/squaregraph.tex <==


%% Cycle, based on Tikz example library by Author : Jerome Tremblay

\begin{tikzpicture}

\def \n {5}
\def \radius {2cm}
\def \margin {10pt} % margin in angles, depends on the radius



\def \nm {\numexpr(\n-1)\relax}  %n minus one
\def \nmm {\numexpr(\n-2)\relax}  % \n minus minus

\foreach \s in {0,...,\nm}
{
	\node[draw,circle,minimum size=15pt,inner sep=0] (vp\s) at (\s * \radius,\radius) {$v'_{\s}$};
	\node[draw,circle,minimum size=15pt,inner sep=0] (v\s) at (\s * \radius,0) {$v_{\s}$};
	\draw (v\s) -- (vp\s);
}

\foreach \s[count=\sprev from 0] in {1,...,\nm}
{
	\draw (vp\sprev) -- (vp\s);
	\draw (v\sprev) -- (v\s);
}


% C_0
\draw[dashed,->,thick] (0.18*\radius, 0.3*\radius) arc (200:-30:0.35*\radius);
\node at (0.5*\radius,0.5*\radius) {$C_0$};

%E's
\foreach \s[count=\sprev from 1] in {2,...,\nm}
{
	\draw[->,>=latex,blue,dashed,rounded corners]  
		(\sprev* \radius + \margin, \radius -\margin) --
		(\s * \radius - \margin, \radius -\margin) -- node [left,midway] {$E_{\number\numexpr\sprev-1\relax}$}
		(\s * \radius - \margin, \margin) --
		(\sprev * \radius + \margin, \margin);
}

\end{tikzpicture}
